Dimension-free deterministic equivalents and scaling laws for random feature regression

In this work we investigate the generalization performance of random feature ridge regression (RFRR). Our main contribution is a general deterministic equivalent for the test error of RFRR. Specifically, under a certain concentration property, we show that the test error is well approximated by a closed-form expression that only depends on the feature map eigenvalues. Notably, our approximation guarantee is non-asymptotic, multiplicative, and independent of the feature map dimension -- allowing for infinite-dimensional features. We expect this deterministic equivalent to hold broadly beyond our theoretical analysis, and we empirically validate its predictions on various real and synthetic datasets. As an application, we derive sharp excess error rates under standard power-law assumptions of the spectrum and target decay. In particular, we provide a tight result for the smallest number of features achieving optimal minimax error rate.

==> sections/conclusion.tex <==
In this paper, we have investigated the generalization properties of random feature models, deriving a non-asymptotic deterministic equivalent for the risk of random feature ridge regression---which recovers (and unifies) previous asymptotic findings as special limits. Our results provide a rigorous multiplicative approximation rate, enabling us to analyze error scaling laws under source and capacity conditions, and offers a complete view of the different scaling regimes and their cross-overs. 

Our analysis relies on Assumption \ref{ass:concentration_eigenfunctions} which, while popular in theoretical investigations, excludes more realistic random feature models, such as  $\varphi(\bx, \bw) = \sigma(\bx^{\top} \bw)$ with $\bx,\bw$ Gaussian vectors and non-linear $\sigma$. Although restrictive, this assumption allowed us to derive tight multiplicative approximation bounds for a generic random feature model with infinite-dimensional features---which was essential for obtaining the rigorous excess risk rates that are the primary motivation of our work.
We further note that numerical simulations in Figure \ref{fig:examples} and Appendix \ref{app:numerics} suggest that the predictions of \Cref{thm:main_test_error_RFRR} remain accurate much beyond Assumption \ref{ass:concentration_eigenfunctions}. We consider lifting this technical condition---e.g., by following the approach in \cite{misiakiewicz2024nonasymptotic}---to be an important direction for future research. 
